HETFORMER: Heterogeneous Transformer with Sparse Attention for Long-Text Extractive Summarization

To capture the semantic graph structure from raw text, most existing summarization approaches are built on GNNs with a pre-trained model. However, these methods suffer from cumbersome procedures and inefficient computations for long-text documents. To mitigate these issues, this paper proposes HETFORMER, a Transformer-based pre-trained model with multi-granularity sparse attentions for long-text extractive summarization. Specifically, we model different types of semantic nodes in raw text as a potential heterogeneous graph and directly learn heterogeneous relationships (edges) among nodes by Transformer. Extensive experiments on both single- and multi-document summarization tasks show that HETFORMER achieves state-of-the-art performance in Rouge F1 while using less memory and fewer parameters.

==> 02_REL.tex <==
\section{Background}

\subsection{Graph-enhanced Summarization}
In the recent state-of-the-art summerization models, there is a trend to extract the structure from the text to formulate the document text as hierarchical structure or heterogeneous graph. \textit{HiBERT}~\citep{zhang2019hibert}, \textit{GraphSum}~\citep{li2020leveraging} and \textit{HT}~\citep{liu2019hierarchical} consider the word-level, sentence-level and document-level of the input text to formulate the hierarchical structure. \textit{MGSum}~\citep{hanqi2020granularity}, \textit{ASGARD}~\citep{huang2020knowledge}, \textit{HSG}~\citep{wang2020heterogeneous} and  \textit{HAHSum}~\citep{jia2020neural} construct the source article as a heterogeneous graph where words, sentences and entities are used as the semantic nodes and they iteratively update the sentence nodes representation which is used to do the sentence extraction.

% \textit{ASGARD}~\citep{huang2020knowledge} constructs a homogeneous knowledge graph SEG-graph from an input document, which contains the entity and relation information and a homogeneous document graph DOC-graph which only contains text. The DOC-graph focuses on the global context and SEG-graph captures topic shift among the entities. \textit{HSG}~\citep{wang2020heterogeneous} proposes a heterogeneous graph network where words and sentences are used as the semantic nodes and they iteratively update the sentence nodes representation which is used to do the sentence extraction. \textit{HAHSum}~\citep{jia2020neural} construct the source article as a heterogeneous graph which can be viewed as two-level graph: word-level and sentence-level. The word-level subgraph contains word and entity. 

The limitation of those models is that they use pre-trained methods as the feature-based model to learn the node feature and build which brings more training parameters than just using pre-trained methods. So compare with those models, our work can achieve the same thing but using the lite framework.
Moreover, these models typically limit inputs to $n=512$ tokens since the $O(n^{2})$ cost of attention. Due to the long source article, when applying BERT or RoBERTa to the summarization task, they need to truncate source documents into one or several smaller block input~\citep{li2020leveraging,jia2020neural,huang2020knowledge}.

\subsection{Structure Transformer with Sparsity}
% There are four categories to scale up attention to the long input: sparse attention, recurrence~\citep{dai2019transformer,katharopoulos2020transformers}, hierarchical mechanisms~\citep{zhang2019hibert} and compressed attention~\citep{maruf2019selective}. Since our work is most related to the sparse attention, we will just discuss sparse attention here. Sparse attention involves limiting each token to attend to a subset of the other tokens. For example, the \textit{Sparse Transformer}~\citep{child2019generating} used predefined attention patterns for both text and image generation. They showed that attending only to previous pixels in the same row or column was enough to generate high quality images, while keeping attention cost at $O(n\sqrt{n})$. The \textit{Reformer} model~\citep{kitaev2020reformer} finds the nearest neighbors of the attention query using locality sensing hashing~\citep{andoni2015practical} and only uses those for attention. This reduces attention cost to $O(n\log{n})$. The \textit{Clustered Transformer}~\citep{vyas2020fast} introduces clustered attention by first extracting the top-k keys with the highest attention per cluster and then computing the attention on these keys separately for each query that belongs to the cluster. Finally, 
The most related approaches to the work presented in this paper are
\textit{Longformer}~\citep{beltagy2020longformer} and \textit{ETC}~\citep{ravula2020etc} which feature a very similar global-local attention mechanism and take advantage of the pre-trained model RoBERTa. Except Longformer has a single input sequence with some tokens marked as global (the only ones that use full attention), while the global tokens in the ETC is pre-trained with CPC loss. Comparing with those two works, we formulate the heterogeneous attention mechanism, which can consider the word-to-word, word-to-sen, sen-to-word and entity-to-entity attention. 

\subsection{Graph Transformer}
With the great similarity between the attention mechanism used in both Transformer \citep{vaswani2017attention} and Graph Attention network~\citep{velivckovic2017graph}, there are several recent Graph Transformer works recently. Such as GTN~\citep{yun2019graph}, HGT~\citep{hu2020heterogeneous}, HetGT~\citep{yao2020heterogeneous} formulate the different type of the attention mechanisms to capture the node relationship in the graph.

The major different between of our work and Graph Transformer is that the input of graph transformer is structural input, such as graph or dependence tree, but the input of our HeterFormer is unstructured text information. 
Our work is to convert the transformer to structural structure so that it can capture the latent relation in the unstructured text, such as the word-to-word, word-to-sent, sent-to-word, sent-to-sent and entity-to-entity relations. 

% Besides, to capture the structural input, graph transformer incorporates the relation information. 

% 1. those works trend to using BERT or RoBERTa as the feature-based method to first initial the node embedding and then use the GNN on top of the BERT to model as the heterogeneous network to message passing the information and structural learn the representation of node and do the extractive summarization. 
% 2. we argue that our work is 
% Compare with the heterogeneous graph works, our work can do the same thing as the 
